Autonomous Drifting with 3 Minutes of Data via Learned Tire Models

Near the limits of adhesion, the forces generated by a tire are nonlinear and intricately coupled. Efficient and accurate modelling in this region could improve safety, especially in emergency situations where high forces are required. To this end, we propose a novel family of tire force models based on neural ordinary differential equations and a neural-ExpTanh parameterization. These models are designed to satisfy physically insightful assumptions while also having sufficient fidelity to capture higher-order effects directly from vehicle state measurements. They are used as drop-in replacements for an analytical brush tire model in an existing nonlinear model predictive control framework. Experiments with a customized Toyota Supra show that scarce amounts of driving data -- less than three minutes -- is sufficient to achieve high-performance autonomous drifting on various trajectories with speeds up to 45mph. Comparisons with the benchmark model show a $4 \times$ improvement in tracking performance, smoother control inputs, and faster and more consistent computation time.

==> tex/02_related_work.tex <==

\noindent {\textbf{Related work.}
A plethora of tire models~\cite{PACEJKA2012xiii,Svendenius2003ConstructionON, svendenius2007tire, Acosta2017TireLF,Guarneri2008ANM, Xu2022TireFE, Matuko2008NeuralNB} has been proposed in the literature. We consider as a baseline model the Magic Formula \cite{PACEJKA2012xiii}, predominantly used in industry. Black-box or Magic Formula-based neural network models~\cite{Acosta2017TireLF,Guarneri2008ANM, Xu2022TireFE, Matuko2008NeuralNB} have also been proposed. However, these models do not retain the physics-based guarantees and none has been tested on a full-size car operating at the limits of handling.

Autonomous drifting and racing have been successfully performed in previous work~\cite{Goh2019TowardAV,balachandran2023human,Hindiyeh2011ACF,Subosits2021ImpactsOM,Goh2016SimultaneousSA,Spielberg2019NeuralNV}. In these approaches, the Fiala brush model~\cite{fiala1954seitenkraften} is often used due to its efficient balance between accuracy and simplicity. Our experiments show that both NODE and \texttt{ExpTanh} models have the potential to outperform the Fiala brush model on several metrics.
}
